Approximate Linear Programming for Decentralized Policy Iteration in Cooperative Multi-agent Markov Decision Processes

In this work, we consider a cooperative multi-agent Markov decision process (MDP) involving m agents. At each decision epoch, all the m agents independently select actions in order to maximize a common long-term objective. In the policy iteration process of multi-agent setup, the number of actions grows exponentially with the number of agents, incurring huge computational costs. Thus, recent works consider decentralized policy improvement, where each agent improves its decisions unilaterally, assuming that the decisions of the other agents are fixed. However, exact value functions are considered in the literature, which is computationally expensive for a large number of agents with high dimensional state-action space. Thus, we propose approximate decentralized policy iteration algorithms, using approximate linear programming with function approximation to compute the approximate value function for decentralized policy improvement. Further, we consider (both) cooperative multi-agent finite and infinite horizon discounted MDPs and propose suitable algorithms in each case. Moreover, we provide theoretical guarantees for our algorithms and also demonstrate their advantages over existing state-of-the-art algorithms in the literature.

==> convergence.tex <==
     
  \section{Theoretical Analysis}
  



==> relatedworks.tex <==
\section{Related Work}
\label{relatedWork}
In the literature, policy and value iteration techniques have been largely well-studied in the context of SA-MDP \cite{bertsekas2017}, \cite{puterman}.  Further, ALP approaches have been well studied in the SA-MDP setting \cite{desai2012, malek2014, CLSBCS}. One of the key challenges when using LP-based techniques is the large number of constraints. This problem is tackled in \cite{CLSBCS} through reduction via a linearly relaxed ALP with lower number of constraints obtained from taking a positive linear combination of the original constraints. However, in this paper, 
our focus is on approximate linear programming (ALP) approaches in the context of MA-MDP. 

Our paper aims to develop ALP-based algorithms for the MA-MDP setting using a decentralized setup to enhance computational efficiency. Many recent works have aimed to tackle problems in the domain of MA-MDP, many of which focus on the cost reduction task as it is one of the most critical problems in this domain. 
Many algorithms have been proposed in the literature to resolve this issue. Further, in the MA-MDP setting, the associated cost and computational complexity increase with the number of agents. We briefly discuss some of the works in the literature that address the issue of cost reduction in MA-MDP.

In \cite{Nawaz_2023}, the authors employed MA-MDP for multi-target path planning. Agents in autonomous systems are frequently required to visit multiple targets under complex operating conditions. The authors considered a non-communicating setup of MA-MDP where agents need to visit a set of targets in minimum time. The authors then propose a heuristic partitioning procedure to solve the MA-MDP, attempting to solve the $m$-TSP (i.e., Transportation Service Provider) on the model graph and show that their approach generates an optimal partition for clustered target states. However, they did not consider a cooperative MA-MDP setup with decentralized policy improvement. In \cite{Peng_2019}, policy iteration is used in communicating multi-agent optimal tracking control. A data-driven approach is used together with a neural network to approximate  both the iterative control laws and the iterative performance index functions. However, decentralized policy iteration in the MA-MDP setup is not considered.

In \cite{bertsekas_VI_2020}, multi-agent value iteration (VI) for an infinite horizon setting is considered. Since this is a multi-agent setting, at each stage, the control consists of multiple distinct decisions made by one of several agents. Here, value iteration algorithms consider component-by-component minimization, unlike simultaneous minimization of all components at each stage, and the value iteration procedure is presented for more general dynamic programming settings, where the Bellman operator is a contraction mapping. The agent-by-agent implementation of the VI algorithm reduces computational requirements over regular VI, which may be computationally intractable even for a moderate number of agents. On the other hand, such algorithms may terminate with a sub-optimal policy, which may still be agent-by-agent optimal. However, unlike our work, approximate VI is not discussed in that work.

In \cite{Bertsekas2021,bertsekas2020}, roll-out and policy iteration using dynamic programming for model-based cooperative multi-agent reinforcement learning are discussed and demonstrate the dynamic programming approach to get the optimal policy starting from a certain base policy. In this work, policy iteration is viewed as a repeated roll-out (the improved policy) implementation in a fully observable MA-MDP system. In this work, the author shows that the required number of computations grows linearly with the number of agents. However, the implementation results of the demonstrated approaches are not presented. Further, approximate decentralized policy improvement is not discussed and implemented.

